On exact relations for the calculation of effective properties of composite

Numerous exact relations exist that relate the effective elastic properties of composites to the elastic properties of their components. These relations can not only be used to determine the properties of certain composites, but also provide checks on the accuracy on numerical techniques for the calculation of effective properties. In this work, some exact relations are discussed and estimates from finite element calculations, the generalized method of cells and the recursive cell method are compared with estimates from the exact relations. Comparisons with effective properties predicted using exact relations show that the best estimates are obtained from the finite element calculations while the moduli are overestimated by the recursive cell method and underestimated by the generalized method of cells. However, not all exact relations can be used to make such a distinction.

==> references.tex <==
\begin{thebibliography}{xx}

\bibitem{Aboudi}{1996}{Aboudi96-1}
Aboudi, J.  ( 1996) , `Micromechanical analysis
  of composites by the method of cells - update', {\em Appl. Mech. Rev} {\bf
  49}(10),~S83--S91.

\bibitem{Banerjee \harvardand\ Adams}{2002{\em a}}{Banerjee02b}
Banerjee, B. \harvardand\ Adams, D.~O.  ( 2002{\em
  a}) , Application of the generalized method of cells to
  polymer bonded explosives.
\newblock To be published.

\bibitem{Banerjee \harvardand\ Adams}{2002{\em b}}{Banerjee02a}
Banerjee, B. \harvardand\ Adams, D.~O.  ( 2002{\em
  b}) , Effective elastic moduli of polymer bonded explosives
  from finite element simulations.
\newblock To be published.

\bibitem{Banerjee \harvardand\ Adams}{2002{\em c}}{Banerjee02c}
Banerjee, B. \harvardand\ Adams, D.~O.  ( 2002{\em
  c}) , On predicting the effective elastic properties of
  polymer bonded explosives using the recursive cell method.
\newblock To be published.

\bibitem[Cherkaev et~al.]{Cherkaev, Lurie \harvardand\
  Milton}{1992}{Cherk92}
Cherkaev, A.~V., Lurie, K.~A. \harvardand\ Milton, G.~W.  (
  1992) , `Invariant properties of the stress in plane
  elasticity and equivalence classes of composites', {\em Proc. R. Soc. Lond.
  A} {\bf 438}(1904),~519--529.

\bibitem[Helsing et~al.]{Helsing, Milton \harvardand\
  Movchan}{1997}{Helsing97}
Helsing, J., Milton, G.~W. \harvardand\ Movchan, A.~B.  (
  1997) , `Duality relations, correspondences, and numerical
  results for planar elastic composites', {\em J. Mech. Phys. Solids} {\bf
  45}(4),~565--590.

\bibitem{Hill}{1964}{Hill64}
Hill, R.  ( 1964) , `Theory of mechanical
  properties of fibre-strengthened materials: I. elastic behaviour', {\em J.
  Mech. Phys. Solids} {\bf 12},~199--212.

\bibitem{Milton}{1997}{Milton97}
Milton, G.~W.  ( 1997) , Composites : a myriad
  of microstructure independent relations, {\em in} T.~Tatsumi, E.~Watanabe
  \harvardand\ T.~Kambe, eds, `Theoretical and Applied Mechanics (Proc. XIX
  International Congress of Theoretical and Applied Mechanics, Kyoto, 1996)',
  Elsevier, Amsterdam, pp.~443--459.

\bibitem{Milton}{2002}{Milton02}
Milton, G.~W.  ( 2002) , {\em Theory of
  Composites}, Cambridge University Press, New York.

\end{thebibliography}

